Measurement of the muon flux for the SHiP experiment

The SHiP experiment will search for very weakly interacting particles beyond the Standard Model which are produced in a 400 \GeV/$c$ proton beam dump at the CERN SPS. About $10^{11}$ muons per spill will be produced in the dump. To design the experiment such that the muon-induced background is minimized, a precise knowledge of the muon spectrum is required. To validate the muon flux generated by our Pythia and GEANT4 based Monte Carlo simulation (FairShip), we have measured the muon flux emanating from a SHiP-like target at the SPS. This target, consisting of 13 interaction lengths of slabs of molybdenum and tungsten, followed by a 2.4 m iron hadron absorber was placed in the H4 400~\GeV/$c$ proton beam line. To identify muons and to measure the momentum spectrum, a spectrometer instrumented with drift tubes and a muon tagger were used. During a three-week period a dataset for analysis corresponding to $(3.27\pm0.07)~\times~10^{11}$ protons on target was recorded. This amounts to approximatively 1\% of a SHiP spill.

==> Acknowledgments.tex <==
\section{Acknowledgments}
%-- SHiP Acknowledgments as of 9 Nov 2018
%-- 
The SHiP Collaboration acknowledges support from the following Funding Agencies: the National Research Foundation of Korea 
(with grant numbers of 2018R1A2B2007757, 2018R1D1A3B07050649, 2018R1D1A1B07050701, 2017R1D1A1B03036042, 
2017R1A6A3A01075752, 2016R1A2B4012302, and 2016R1A6A3A11930680);  the Russian Foundation for Basic Research (RFBR, grant 17-02-00607) and the TAEK of Turkey.


We thank M. Al-Turany, F. Uhlig. S. Neubert and A. Gheata their assistance with FairRoot. We acknowledge 
G. Eulisse and P.A. Munkes for help with Alibuild.


The measurements reported in this paper would not have been possible 
without a significant financial contribution from CERN. In addition, several member institutes 
made large financial and in-kind contributions to the construction of the target and the 
spectrometer sub detectors, as well as providing expert manpower for commissioning, data 
taking and analysis. This help is gratefully acknowledged. 


